Phenomenology of the minimal B-L extension of the Standard Model at the LHC

A well-motivated framework to naturally introduce neutrino masses is the B-L model, a U(1) extension of the standard model related to the baryon minus lepton gauged number. Besides three right-handed neutrinos, that are included to cancel the anomalies (thereby naturally providing neutrino masses), this model also encompasses a complex scalar for the spontaneous symmetry breaking of the extended gauge sector and to give mass to the Z' boson. We present the phenomenology, the discovery potential at the LHC, and the most up-to-date experimental and theoretical limits of the new particles in this model.

==> Chapter4/chapter4_old.tex <==
\chapter{Phenomenology}\label{Ch:4}
\ifpdf
    \graphicspath{{Chapter4/Chapter4Figs/PNG/}{Chapter4/Chapter4Figs/PDF/}{Chapter4/Chapter4Figs/}}
\else
    \graphicspath{{Chapter4/Chapter4Figs/EPS/}{Chapter4/Chapter4Figs/}}
\fi

In this chapter we study the phenomenology at LHC of the new particles in the pure $B-L$ model. We present the results of our investigation in each sector, with particular emphasis on the gauge and fermionic sectors.

We start with the gauge sector (section~\ref{sect:Zp}), where the properties of the $Z'$ boson (i.e., production cross-sections, intrinsic width, BRs) are delineated.
%, with emphasis on the differences with the traditional literature.
Among them, the possible decay into pairs of heavy neutrinos is certainly the most promising. Finally, a parton level discovery potential and exclusion power studies at the LHC are presented in section~\ref{subsect:disc_power}.

In section~\ref{sect:nu_h} are presented the properties of the fermion sector, i.e., width and BRs of the heavy neutrinos. The possibility for them to be long-lived particles is rather interesting, allowing for signatures with distinctive displaced vertices, in which a high energetic and isolated pair of leptons points to a different vertex than the primary one. Bringing pieces together, the full signature $pp \to Z' \to \nu_h \nu_h$ is studied. In particular, we show that a suitable and peculiar signature to investigate is the tri-lepton decay of the $Z'$ via heavy neutrino pair production. This signature provides a powerful insight in the fermionic sector of the model (and in its interplay with the gauge sector), as it allows for the measure of the heavy neutrino masses. It is remarkable that with the simultaneous measure of the neutrino lifetime (through the displacement of its decay) and mass, light neutrino masses can be inferred.
For a benchmark point, in section~\ref{subsect:trilep} we present a detailed study of the tri-lepton signature (the main result of this Thesis), where signal and backgrounds are fully simulated and analysed (at the parton level and at the detector level), showing that it holds a good signal over background ratio that makes it observable at the LHC, especially as rather generic cuts for background rejection are considered.

Finally, the properties of the scalar sector are delineated in section~\ref{sect:Higgs} (i.e., production cross-sections, intrinsic widths, BRs), where the capabilities for discovery at the LHC are summarised. The main focus is on the impact of the gauge and fermionic sectors. In fact, although no new production mechanisms arise, the decay patterns in this model are rather peculiar, such as the decay into pairs of $Z'$ boson and into heavy neutrinos (besides the decay of the heavy Higgs into pairs of the light scalar bosons). Cross sections for some full processes are presented in section~\ref{subsect:event_rates}.


\section{Gauge sector: $Z'$}\label{sect:Zp}
Differences with other models
\subsection{Production cross sections and decay properties}\label{sect:Zp_properties}
\subsection{Discovery power at the LHC}\label{subsect:disc_power}

The study we present in this paper has been performed using the CalcHEP package \cite{calchep}. The model 
under discussion had been implemented in this package using the 
LanHEP tool \cite{lanhep}, as already discussed in Ref.~\cite{bbms}. 
%The analysis we will provide in the following makes use of subtleties we explicit in the present section. Those that are not common will be explicitly addressed to the place where they have been used.\\

The process we are interested in is di-lepton production. We define our signal as $pp\rightarrow \gamma,\,Z,\,Z'_{B-L}\rightarrow  \ell^+ \ell^-$ ($\ell=e,\,\mu$), i.e., all possible sources together with their mutual interferences, and the background as $pp\rightarrow \gamma,\,Z\rightarrow \ell^+ \ell^-$ ($\ell=e,\,\mu$), i.e., SM Drell-Yan production (including interference). No other sources of background, such as $WW$, $ZZ$, $WZ$ or $t\overline{t}$ have been taken into account. These can be suppressed or/and are insignificant \cite{Ball:2007zza}.
%, by considering adequate cuts and isolation requirements, down to the few percent level}.
For both the signal and the background, we have assumed standard
acceptance cuts (for both electrons and muons) at the LHC:
\begin{equation}\label{LHC_cut}
p_T^\ell > 10~{\rm GeV},\qquad |\eta^\ell|<2.5\qquad (\ell=e,\,\mu),
\end{equation} 
and we apply 
the following requirements on the di-lepton invariant mass,  $M_{ll}$, depending on whether we are considering electrons or muons.
We distinguish two different scenarios: an ``early'' one (for $\sqrt{s}=7$, $10$ TeV) and an ``improved'' one  (for $\sqrt{s}=14$ TeV), and, in computing the signal significances, we will select a window as large as either one width of the $Z'_{B-L}$ boson or twice the di-lepton mass resolution\footnote{We take  the CMS di-electron and di-muon mass resolutions \cite{CMSdet,Ball:2007zza} as a typical LHC environment. ATLAS resolutions \cite{ATLASdet} do not differ substantially.}, 
whichever the largest. The half windows in the invariant mass distributions respectively read, for the ``early scenario'':
\begin{eqnarray}\label{LHC_ris_el}
\mbox{electrons: }\; |M_{ee}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.02\frac{M_{Z'}}{\rm GeV} \right) {\rm GeV}\; \right),\\ \label{LHC_ris_mu}
\mbox{muons: }\; |M_{\mu\mu}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.08\frac{M_{Z'}}{\rm GeV} \right) {\rm GeV}\; \right),
\end{eqnarray}
and for the ``improved scenario'':
\begin{eqnarray}\label{LHC_ris_el_imp}
\mbox{electrons: }\; |M_{ee}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.005\frac{M_{Z'}}{\rm GeV} \right) {\rm GeV}\; \right),\\ \label{LHC_ris_mu_imp}
\mbox{muons: }\; |M_{\mu\mu}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.04\frac{M_{Z'}}{\rm GeV} \right) {\rm GeV}\; \right).
\end{eqnarray}
Our choice reflects the fact that what we will observe is in fact the convolution 
between the Gaussian detector resolution and the Breit-Wigner 
shape of the peak, and such convolution will be dominated by the largest of the two. Our approach is to take the convolution width exactly equal to the resolution width or to the peak width, whichever is largest, and to count all the events within this window. Finally, only $68\%$ of signal events are considered: intrinsically, when the the peak width is dominating, effectivelly (by rescaling the signal), otherwise.

In figure \ref{CMS_res} we compare the LHC resolutions for electrons for the two aforementioned scenarios (eqs.~(\ref{LHC_ris_el}) and (\ref{LHC_ris_el_imp})) with $\Gamma_{Z'}/2$.
It is clear that, whichever the $Z'_{B-L}$ mass, for a value of the coupling $g'_1$ smaller than roughly $0.4$, the peak will be dominated by the early experimental resolution,
%
%
%
%\footnote{To guarantee a smooth transition between the two regimes ($\Gamma _{Z'}/2 \ll \sigma$ and $ \Gamma _{Z'}/2 \gg \sigma$), we decided to linearly interpolate the region $ \sigma /3 < \Gamma _{Z'}/2 < \sigma$, as in the first regime making the convolution implies to consider just the $68\%$ of the signal, while in the second regime all the generated signal is taken. This procedure effectively pushes down the value of the coupling for which the transition occurs ($g'_1 \sim 0.1\div 0.2$) and the two considered channels give equal results. Anyway, regardless of the regime, this procedure implies that always the $68\%$ ($70\%$ in the width-dominated regime) of the signal is considered.\label{footnote_equiv}}
i.e., the half window 
will contain an amount of signal as big as the one produced with
$|M_{ll}-M_{Z'}| = \Gamma_{Z'}/2$. The region of interest in the parameter space we are going to study almost always fulfils the condition $g'_1<0.4$, as we will
see from the plots in the following section. The muon resolution is much worse and in such a plot it would be an order of magnitude higher than the other curves. Hence, for this final state, the peak is always dominated by the experimental resolution, for the values of the gauge coupling we are considering.

\begin{figure}[!h]
  \includegraphics[angle=0,width=0.8\textwidth ]{figures/CMS_res_corr.eps}
  \caption{\it Comparison of the CMS electron resolution according to eqs.~(\ref{LHC_ris_el}) and (\ref{LHC_ris_el_imp}), with the two different constant terms as described in the text, compared to $\, \Gamma _{Z'}/2$ for $g'_1=0.23$ and $g'_1=0.44$.}
  \label{CMS_res}
\end{figure}

In the next section we will compare the LHC and Tevatron discovery reach. For the latter, we have considered typical acceptance cuts (for both electrons and muons):
\begin{equation}\label{Tev_cut}
p_T^\ell > 18~{\rm GeV},\qquad |\eta^\ell|<1\qquad (\ell=e,\,\mu),
\end{equation}
and the following requirements on the di-lepton invariant mass,  $M_{ll}$, depending on whether we are considering electrons or 
muons\footnote{We take the CDF di-electron and di-muon mass resolution \cite{CDFdet} as a typical Tevatron environment.}:
\begin{eqnarray}\label{Tev_ris}
\mbox{electron: }\; |M_{ee}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.135 \sqrt{\frac{M_{Z'}}{\rm GeV}}{\rm GeV}+ 0.02\frac{M_{Z'}}{\rm GeV} \right) {\rm GeV}\; \right),\\
\mbox{muons: }\; |M_{\mu\mu}-M_{Z'}| &<& 
\mbox{max} \left( \frac{\Gamma_{Z'}}{2},\; \left( 0.0005\left(\frac{M_{Z'}}{2\, \rm GeV}\right) ^2 \right) {\rm GeV}\; \right).
\end{eqnarray}


The selection of an invariant mass window centered at the $Z'$ boson mass is comparable to the standard experimental analysis, as in Ref.~\cite{D0} (the electron channel at $D\varnothing$), where signal and background are integrated from $M_{Z'}-3\Gamma _{Z'}$ (where $\Gamma _{Z'}$ is the $Z'$ boson width obtained by rescaling the SM-$Z$ boson width by the ratio of the $Z'$ to the $Z$ boson mass) to infinity. Effectively, the integration stops close to $M_{Z'}+3\Gamma _{Z'}$. Since the background can be reasonably thought as flat, while the signal is not, the procedure we propose enhances the signal more than the background and it is expected to be more sensitive. Although the first reference of~\cite{Tevatron_bounds} applies a different strategy, figure~\ref{contour7_ecal} shows that our procedure could improve recent constraints. The performance of our procedure is similar to the analysis of the second reference of Ref.~\cite{Tevatron_bounds} (the muon channel), although less involved. Notice, also, that, regarding the CDF detector, the efficencies for reconstructing electrons and muons are similar (see Ref.~\cite{Abulencia:2005ix} for an analysis at the $Z$ peak).
At the LHC. it is being discussed to implement a completely different approach, based on a line-shape fit. Hence, we present our results for a late comparison.


In our analysis we use a definition of signal significance $\sigma$, as follows. 
In the region where the number
of both signal ($s$) and background ($b$) 
events is ``large'' (here taken to be bigger than 20),
we use a definition of significance
based on Gaussian statistics:
\begin{equation}
{\sigma} \equiv {\it s}/{\sqrt{\it b}}.
\end{equation}
Otherwise, in case of smaller statistics,
we used the 
Bityukov algorithm \cite{Bityukov}, which basically uses the 
Poisson `true' distribution instead of the approximate Gaussian one.

Finally, as in \cite{bbms,bbmp}, we used {\rm{CTEQ6L}} \cite{CTEQ} as default Parton Distribution Functions (PDFs), evaluated at the scale $Q^2=M_{ll}^2$.
The leading order (LO) cross sections are multiplied by a mass independent $k-$factor of $1.3$ \cite{Carena} (for the cross sections evaluated at the Tevatron), as in Refs.~\cite{Tevatron_bounds,D0}, or $1.35$ (for the cross sections evaluated at the LHC), as in Ref.~\cite{Ball:2007zza}\footnote{We are aware that the use of different values could be inconsistent. The variation is anyway very small and the results do not change substantially with the chosen value.}, to get in agreement with the Next-to-Next-to-Leading-Order (NNLO) QCD corrections.

Typical detector resolution has effectively been taken into account by our procedure, that consists in counting all the events that occur within the window (in invariant mass) previously described, and by rescaling to $68\%$ the signal events when the peak is dominated by the experimental resolution.
Nonetheless, our simulation does not account for Initial State Radiation (ISR) effects. 
%Regarding  the former, their impact is to broaden the peaks, however, in case of resolution dominated peaks (in which all the $Z'$ resonance is 
%essentially contained within the experimental resolution), no changes in the significance will occur; otherwise the effect will tend to deplete somehow the signal rates, but only for very high $Z'$ masses and large $B-L$ gauge couplings (at the margin of our parameter space).
ISR can have two main sources: QED-like ISR (i.e., photon emission), that has the effect of shifting the peak and of creating a tail towards smaller energy, and QCD-like ISR (i.e., gluon emission), that has similar effects and might also induce trigger issues
%if jets are cut from the final state (e.g., with
in the intent of removing backgrounds (e.g., by cutting on final state jets). Although we are aware of such effects, we believe that their analysis goes beyond the scope of this paper and it will be reported on separately \cite{preparation}. Altogether, we are confident that, while particular aspects of
our analysis may be sensitive to such effects, the general picture will not depend upon these substantially (see section~\ref{validation}).
%The only comment we would like to make here is that including ISR, even if no hard jet are asked to appear in the final state, will enhance the total cross-section for our signal, by a factor $40\%$-$50\%$ depending on the $p_T$ cut in the trigger. As we will show later on, our zone-of-interest in the $M_{Z'}-g'_1$ plane is such that the background is always negligible and the signal barely visible. Given that, we can claim that the results we give here can be considered as conservative, even if we do just a parton level analysis.
Also, the only background considered here was the irreducible SM Drell-Yan. Reducible backgrounds, photon-to-electron conversion, efficiencies in reconstructing electrons/muons, jets faking leptons etc., whose overall effect is to deplete the signal, were neglected (being $t\overline{t}$ the most important source, at the level of $ \lesssim 10\%$). However, for this analysis they are not quantitatively important \cite{Abulencia:2005ix,Ball:2007zza}.
%although they need to be taken into account for a more refined analysis.


\subsubsection{LHC at $\sqrt{s}=7$ TeV and comparison with Tevatron}
\subsubsection*{Exclusion power}
\subsubsection{LHC at $\sqrt{s}=14$ TeV}
\subsubsection*{Exclusion power}

\section{Heavy neutrinos}\label{sect:nu_h}
\subsection{Production cross sections and decay properties}\label{sect:nu_properties}
\subsection{$pp\to Z'\to \nu_h \nu_h$ phenomenology}
\subsection{Tri-lepton signature analysis (parton level vs. detector level)}\label{subsect:trilep}
\subsubsection{Parton level}
\subsubsection{Detector level}

\section{Higgs}\label{sect:Higgs}
\subsection{Production cross sections and decay properties}
focus on $Z'$ and neutrinos
\subsection{Cross sections for processes involving $Z'$ and neutrinos}\label{subsect:event_rates}


==> Macros/MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 

